Diversified Dynamic Routing for Vision Tasks

Deep learning models for vision tasks are trained on large datasets under the assumption that there exists a universal representation that can be used to make predictions for all samples. Whereas high complexity models are proven to be capable of learning such representations, a mixture of experts trained on specific subsets of the data can infer the labels more efficiently. However using mixture of experts poses two new problems, namely (i) assigning the correct expert at inference time when a new unseen sample is presented. (ii) Finding the optimal partitioning of the training data, such that the experts rely the least on common features. In Dynamic Routing (DR) a novel architecture is proposed where each layer is composed of a set of experts, however without addressing the two challenges we demonstrate that the model reverts to using the same subset of experts. In our method, Diversified Dynamic Routing (DivDR) the model is explicitly trained to solve the challenge of finding relevant partitioning of the data and assigning the correct experts in an unsupervised approach. We conduct several experiments on semantic segmentation on Cityscapes and object detection and instance segmentation on MS-COCO showing improved performance over several baselines.

==> figures/ablation-alpha-segmentation.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/ablation-alpha-segmentation_.pdf}
    \caption{Ablation on the $\alpha$ parameter of the diversity loss term.
    We can see that the method is stable regardless the choice of $\alpha$.
    }
    \label{fig:ablation-alpha-segmentation}
\end{figure}

==> figures/ablation-lambda2-detection.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\textwidth]{figures/ablation-lambda2-detection_.pdf}
    \caption{Ablation on the $\lambda_2$ parameter of the diversity loss term.
    We can see that the method is stable in terms of accuracy and model complexity as the regularization term $\lambda_2$ stays in a reasonable range.
    Apart from that, the training is less sensitive to the strength of the regularization.
    }
    \label{fig:ablation-alpha-segmentation}
\end{figure}

==> figures/car-area-per-image.tex <==
\begin{figure}[ht]
    \label{fig:car-area-per-image}
    \centering
    \includegraphics[width=.8\textwidth]{figures/car-area-per-image_.pdf}
    \caption{
        Statistics of car instances per images in the training dataset,
        where the X-axis represents horizontal location of the center of the objects.
    }
\end{figure}


==> figures/cityscapes-splice.tex <==
\begin{figure}[t]
    \label{fig:cityscapes-splice}
    \centering
    \includegraphics[width=.8\textwidth]{figures/cityscapes-slice_.pdf}
    \caption{
        We manually pick two horizontal slicing axes that we use
        to slice the original training and the validation set of
        Cityscapes~\cite{cordts2016cityscapes}.
        We apply the same coordinates over all the samples in the
        dataset.
    }
\end{figure}


==> figures/class-specific-nas-accuracy.tex <==
\begin{figure}[ht]
    \label{fig:class-specific-nas-accuracy}
    \centering
    \includegraphics[width=.8\textwidth]{figures/class-specific-nas-accuracy_.pdf}
    \caption{
        Scores are aggregated over 3 different runs with
        identical hyperparameters and varying random seeds.
    }
\end{figure}


==> figures/class-specific-nas-cell-count.tex <==
\begin{figure}[ht]
    \label{fig:class-specific-nas-cell-count}
    \centering
    \includegraphics[width=.8\textwidth]{figures/class-specific-nas-cell-count_.pdf}
    \caption{
        Scores are aggregated over 3 different runs with
        identical hyperparameters and varying random seeds.
        Variance of each reported count is measured over the joint of
        the training and validation set of Cityscapes~\cite{cordts2016cityscapes}.
    }
\end{figure}


==> figures/k-tsne-cityscapes.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.9\textwidth]{figures/k-tsne-cityscapes_.pdf}
    \caption{
        Visualizing the $183$-dimensional $\mathcal{A}$-space with  of models trained on Cityscapes~\cite{cordts2016cityscapes} using t-SNE~\cite{van2008visualizing}. 
        \textit{Left:} varying number of \textit{local experts}, $K=2,3,4$.
        \textit{Right:} joint t-SNE visualization of architectures of Dynamic Routing~\cite{li2020learning} (\textit{orange}) and our approach (\textit{blue}).
        It is clear that our method not only encourages diversity of the learned routes but also reduces variance in a specific cluster.
        Low \textit{intra}-cluster variance is beneficial because it facilitates feature sharing between similar tasks
    }
    \label{fig:k-tsne-cityscapes}
\end{figure}

==> figures/meaningful-subset.tex <==
\begin{figure}
    \centering
    \includegraphics[width=.8\textwidth]{figures/meaningful-subset_.pdf}
    \caption{
        A single dataset can be split-up into subsets in multiple ways, each resulting in a set of \textit{local experts}.
        In Section \ref{sec:motivation} we have shown when subsets have substantial differences, the corresponding architectures are also unique to the subsets.
        Using this insight, we use the architecture space $\mathcal{A}$ to assign the training data to subsets that maximize the distances between the resulting \textit{local experts}
    }
    \label{fig:subset}
\end{figure}

==> figures/nas-vs-dr.tex <==
% \begin{figure*}[t]
%     \label{fig:nas-vs-dr}
%     \centering
%     \includegraphics[width=\textwidth]{figures/nas-vs-dr_.pdf}
%     \caption{
%         Our hypothesis is that in practice the dataset can be divided into clusters based on their underlying structure i.e. geometry and texture,
%         such that running Neural Architecture Search (NAS) on each individual cluster would result in substantially diverse solutions (middle).figure
%         More than that, under a computational budget constraint, an offline search on the entire dataset will probably result in a sub-optimal solution (left), compared to running cluster-specific search (middle).
%         However, cluster-specific NAS relies on
%         i) a provided clustering of the data and
%         ii) an oracle that assigns each sample to a cluster during inference time.
%         %
%         We propose to utilize Dynamic Routing (DR, right) to
%         i) cluster the data during training time, such that it maximizes the distances between the cluster-specific architectures and
%         % ii) allow us to infer the cluster of an unseen sample in parallel with the actual class-labels.
%         ii) assign the best matching architecture in parallel with the class-label inference for unseen samples.
%     }
% \end{figure*}


==> figures/s-l-x-arch.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\textwidth]{figures/s-l-x-arch-garamond-v2.pdf}
    \caption{
        Local experts (\textit{left} and \textit{middle}) outperform (global experts) (\textit{right}) both in terms of accuracy (Intersection over Union) and computational complexity (Giga Flops).
        In this figure we use the notation of DR~\cite{li2020learning}, namely each row corresponds to processing the previous layer's features on a different resolution (top row corresponds to the highest resolution, bottom row to the lowest).
        Each node represents a convolutional block encapsulated by a gate.
        If a node has no outgoing edges its input is forwarded without transformation
    }
    \label{fig:s-l-x-arch}
\end{figure}

==> figures/subset-arch.tex <==
\begin{figure}[ht]
    \label{fig:subset-arch}
    \centering
    \includegraphics[width=.8\textwidth]{figures/subset-arch_.pdf}
\end{figure}


==> figures/wrapped-fig.tex <==
% \begin{wrapfigure}{r}{0.3\textwidth}
% \begin{figure}
%   \begin{center}
%     \includegraphics[width=0.28\textwidth]{figures/wrapped-fig_.pdf}
%   \end{center}
%   \caption{$\mathcal{A}$ maps inputs to architectures}
%   \label{fig:wrapped-fig}
%   \end{figure}
% \end{wrapfigure}

==> sections/experiments_old.tex <==
\section{Experiments}
\label{sec:experiments}

In this section, we first analyze the \textit{dynamic} property of~\cite{li2020learning} and show that the variance of the gate activation with regards to the input samples are negligible over both training and unseen validation data.
Followed by that, we compare our method against~\cite{li2020learning} in terms of accuracy, computational efficiency and variance of the proposed network layout.
We show that using our proposal we can improve the accuracy while maintaining the same average computational cost.
Lastly, we show strengths and limitations of our method.

\subsection{Implementation Details}
In our experiments we replicated the training environment detailed in~\cite{li2020learning}.
Due to computational constraints we could only reproduce the results of the lower complexity variant the 16 layer Dynamic Routing network using 4xP100 GPUs.
We train models on the Cityscapes~\cite{cordts2016cityscapes} dataset with 2975 training images and 500 images held out for validation.
We do not use the \textit{coarse} annotations, that contains 20k coarsely labeled images.

\textcolor{red}{PASCAL VOC?}

\subsection{Mode collapse in Dynamic Routing}
\label{sec:static-dr}
In our first experiment we asses the dynamic property of DR~\cite{li2020learning}, by training three individual models on small $\mathcal{D}_S$, large $\mathcal{D}_L$ and mixed $\mathcal{D}_X$ scale objects.
We refer to the corresponding architectures $\mathcal{A}_S(x), \mathcal{A}_L(x)$ and $\mathcal{A}_X(x)\in\left[0,1\right]^{183}$ respectively.
To ensure diversity in the results we run 3 independent training at each scale with different random seeds.
Furthermore, we apply the strongest computational-budget regularization from~\cite{li2020learning} (Layer-16, Dynamic-A setting) during training.

To evaluate the variance between the resulting architectures we compute the standard deviation over the samples for each gate output $\sigma\in\left[0,\infty\right)^{183}$ and average it over the gate outputs:
\begin{equation*}
    var(\mathcal{A}, \mathcal{D}) =
    \frac{1}{dim(\mathcal{A})}
    \sum_i\sigma^i_{x\in \mathcal{D}}(\mathcal{A}(x)).
\end{equation*}

% \csabi{This is way too convoluted to be in the main paper, should be just pointed in the appendix maybe?}
In the \textbf{Appendix}, we report the averaged differences across multiple trainings with varying random seed.
From these results, we conclude that the variance of the dynamic architecture in the original formulation of~\cite{li2020learning} is negligible.
From further analysis (see \textbf{Appendix}%~\ref{appendix:static-gate-variance-analysis}
), we learn that the variance is non-zero only due to a limited number of gate activations varying between $\left(0, 1\right)$, but never reaching $0$, where the actual operation would be pruned according to~\cite{li2020learning}.

This means that the computational-efficiency improvement attributed to the dynamic property in~\cite{li2020learning} is only the result of optimizing the budget-constraint during training time, leading to reduced model complexity, but otherwise static architecture: $\frac{\partial}{\partial x}\mathcal{A}=0$.

In the off-diagonal entries of Table~\ref{tab:dr-std} we evaluate the variance over validation sets other than the training set.
This provide further evidence of our claim: the network architecture stays static even when exposed out of distribution samples of the input data.
% \csabi{In theory, it would be still possible that the model recognizes the out of distribution samples and consistently changes the layout for the entirety of the validation set.}

Following the terminology of conditional generative models, we refer to this undesired behaviour as mode collapse in the space of architectures, since the conditional distribution $p(\mathcal{A}|x)$ is practically constant, irrespective of the data $p(\mathcal{A}|x) = p(\mathcal{A})$.
From further on, to remain consistent in our experiments, we reuse $\mathcal{A}_{S,L,X}$ as static architectures.

Although Dynamic Routing fails to map different images to different architecture, training with the budget constraint admits interesting properties, that results in various architectures over different random-initializations.
In the next section, we look at the qualitative and quantitative differences between the learned architectures.

\input{tables/dr-std.tex}

\input{figures/s-l-x-arch.tex}


%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\subsubsection{Comparison of cluster-specific and global NAS}
\label{sec:local-global-nas}
Our hypotheses is that running independent NAS with a computational budget constraint on subsets of a dataset that share the same bias leads to better solutions than searching for a global architecture, both in terms of accuracy and computational complexity.
We test this hypothesis in our toy-experiment, where the subset bias is provided manually by terms of splitting the input images into areas that are more likely to contain smaller $\mathcal{D}_S$ or larger objects $\mathcal{D}_L$.
In the case of global NAS to obtain the training dataset $\mathcal{D}_X$, we sample the images from the two datasets uniformly and discard the scale-information.
We argue that this setup is particularly useful for testing our hypothesis since the search space of DR~\cite{li2020learning} allows inference on multiple resolutions and we expect to see significantly different solutions when NAS is performed on $\mathcal{D}_S$ and $\mathcal{D}_L$.
Therefore, in this section we discuss similarities between models trained on the same scale and differences between architectures corresponding to different scales.
We expect to see the following:
\begin{itemize}
    \item Performing cost-aware NAS on a dataset that contains small-scale objects will result in architectures that omit low-resolution pathways (bottom row of the architecture).
    \item Results on large-scale objects will prefer low-resolution pathways as it enables utilization of more learnable-parameters, than inference on high-resolution, constrained by the same computation budget.
    \item A single dynamic routing model will show similar behaviour after being trained on both small- and large-scale objects.
\end{itemize}


In Figure~\ref{fig:s-l-x-arch} we provide an illustrated example of the results of NAS on each scale, where we also highlight the two most important performance metrics: the accuracy and the computational resource cost.
See the first three rows of Table~\ref{tab:dr-idr-toy} for quantitative comparisons .

\input{tables/dr-idr-toy.tex}

Furthermore, from multiple runs with different random seeds (see \textbf{Appendix}), a pattern reveals: models trained on different scales aligns with the intuition in terms of preferred resolution (downscaling factor is denoted by the side of each row), namely the network L corresponding to large-scale dataset employs more low-resolution cells than the small-scale model S.



%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
%%%%%%%%%%%%%%
\subsubsection{Problem ii: embedding the routing mechanism into the model}
\label{sec:problem-ii}
From the previous experiments we concluded that it is beneficial to run cluster specific architecture search when there is a known significant bias between the subsets of the training data.
In Table~\ref{tab:dr-idr-toy} in the first two rows we only report the metrics on the corresponding validation set, and omit the cross-validation scores to highlight the assumption that both models would be only applied to images from the same distribution as the their respective training set was sampled from.
However this task poses a real challange in practice: during inference time, for each input sample we have to decide which architecture to use.
In order to have an upper-bound on the expected efficiency of Dynamic Routing, we derive a hypothetical setup: \emph{Cluster Specific NAS (CS-NAS) + Oracle},
in which we employ an external \emph{Oracle} model that predicts the subset the new sample belongs to in $c$ FLOPs.
Based on the oracle's prediction we select the corresponding architecture to perform the segmentation.
Given that we operate under a computational budget constraint, $c$ has to be small enough such that we do not lose the advantage of the cost-efficiency of the CS-NAS results.

The naive approach is to train a traditional image classifier using the training data's subset indices as labels, however it makes the setup vulnerable to the mistakes of the Oracle model, since assigning an image to the wrong architecture would lead to inferring the sample with a model trained on a different data distribution.
This vulnerability could be mitigated by finetuning the fixed architectures on the entire training set, however it would compromise the accuracy on the corresponding subset over which the architecture was optimized.

Instead of training an external model, we follow DR~\cite{li2020learning} by considering to reuse the learned representations of the segmentation model at each layer by the \emph{gating mechanism} to select which computational blocks to use in the subsequent layer.
As shown~\cite{li2020learning}, the gates add negligible overhead in terms of FLOPs as they are implemented by two layer fully-connected networks.

In this experiment we provide labels of the subset of the corresponding subset for each training sample, which is taken into account by the Dynamic constraint.
This ensures that the architecture clusters belonging to the two subsets $\mathcal{D}_S$ and $\mathcal{D}_L$ are explicitly incentivized to increase the distance between each other during training. In Table~\ref{tab:dr-idr-toy}, we show how our model performs in terms of accuracy and FLOPs when the subset supervisory signal is available during training.
In the \textbf{Appendix} we illustrate how we measure the alignment of the manual partitioning with the cluster-assignment of Dynamic Routing models:
we infer the validation set and run $k$-means over the resulting architectures with $k=2$,
such that we can use the cluster assignments as predictions of the \emph{Oracle} embedded into the model.
We report the alignment scores in the \textbf{Appendix}.
% Figure~\ref{fig:alignment-progress}.

We conclude that when an external clustering of the dataset is provided, the Dynamic constraint is able to optimize the corresponding architectures jointly.
More than that, we have also shown that the improved DR model is able to recall the most suitable architecture for unseen samples during test time with a high accuracy.
Nevertheless, it is rare that real-life datasets come with handpicked subsets that require different architectures to infer the labels,
thus in our final experiment we will remove the currently assumed subset-supervisory signal, 
to see if the same subsets can be recovered in an unsupervised fashion.

\subsubsection{Problem i: recovering the hidden dataset bias without supervision}
\label{sec:problem-i}
In the final set of experiments on the toy-problem, we evaluate the capabilities of our proposed method to solve \emph{Problem i)}: we show that the manually added dataset-bias can be learned without supervision by the model.

The unsupervised automation of the clustering task is one of the most important claims of our work, since the exhaustive evaluation of every possible partitioning/clustering grows exponentially with the size of the dataset.
On the other hand, dataset biases that are useful from the perspective of the architecture search are scarcely available.
Even on our toy-example, naive evaluation of every possible option is computationally infeasible, since for $K$ number of subsets over $N$ samples one can define $K^N$ unique clustering, which requires in total $K^N\times K$ cluster-specific architecture search.
This motivates our proposal of an iterative approach of jointly optimizing the architecture and clustering the input space.

In the case of the toy-problem, we train our models on the mixed dataset $\mathcal{D}_X$ and expect them to learn the hidden bias, namely the scale variance of objects.
Since we have access to the true subset labels of the underlying images, we can quantify the progress of the \emph{alignment} of the learned clustering with our intuition of how the dataset should be partitioned in a similar fashion as mentioned in Sec~\ref{sec:problem-ii}.
% \csabi{Nevertheless, it is still possible the that the network learns a more useful way to categorize the input samples}

In Table~\ref{tab:dr-idr-toy} we report the performance of the unsupervised variant of our method in terms of accuracy and computational-cost.
In Figure~\ref{fig:alignment-progress} we illustrate the progression of the alignment metric over the training of the unsupervised model.

\input{tables/full-cityscapes-comp}

\subsection{Large scale experiments on Cityscapes}
\label{sec:cityscapes}
After validating our method in a controlled environment, we show the benefits of using the Dynamic constraint in real-world tasks such as the semantic segmentation task of Cityscapes\cite{cordts2016cityscapes}.
In this experiment, we provide \emph{no external supervision} to the Dynamic Routing algorithm about the potential biases in the training dataset. In particular, we compare two version of our proposed unsupervised Dynamic Routing, namely with and without the computational cost constraint. At first, we compare our proposed unsupervised dynamic routing without any computational cost constraints iDR-Raw against the original dynamic routing approach without computational constraint DR-Raw. We observe that while both methods enjoy a similar computational over head of ($116.9$, $115.1$) GFLOPS, our approach $IDR-Raw$ improves the accuracy by $2.3\%$ (from $76.2\%$ to $78.5\%$). On the other hand, when introducing cost efficiency constraint our approach DR-A performs similarly to iDR-A, $74.2$ and $74.0$, respectively with similar computational efficiency. We believe that due to the strong efficiency constraints, this limits the search space for the clusters search. At last, we observe that comparing to other state-of-the-art, our approach, iDR-Raw, performs similarly to DeepLabV3 \cite{chen2017rethinking} with 78.5\% accuracy while performing significantly better in computational efficiency (1778.7GLOPS vs 116.9 GFLOPS).







% In particular, we compare against DR-Raw and DR-A, the dynamic routing approach free from the computational cost constraint and against iDR-A that


% In addition, we compare against several state-of-the-art methods in Table~\ref{tab:full-cityscapes-comp}.

% For example, one could use the metadata such as the location where the input image was taken or the most prominent class on each image as supervisory signals to guide the clustering mechanism.
% Nevertheless, we provide results on the unsupervised variant of our method only, since the availability of such metadata cannot be assumed in general.

% In Table~\ref{tab:full-cityscapes-comp} we provide comparisons with results produced with the official implementation: \href{https://github.com/Megvii-BaseDetection/DynamicRouting}{https://bit.ly/3fY7y3w}.

% We observe that our proposed iDR, without improves over the origi
% We have to note that we could not reproduce the scores reported in the original paper by training models from scratch,
% therefore we report scores using the provided checkpoint files.
% In our experimental setup, we finetune the pretrained models, with identical budget constraints.





% \subsubsection{Ablation studies}
% \input{tables/num-clusters.tex}
% \input{tables/centroid-update.tex}
% \input{tables/img-per-update.tex}

% \input{figures/class-specific-nas-accuracy.tex}
% \input{figures/class-specific-nas-cell-count.tex}

% \subsection{Testing the scale-specific NAS hypothesis}

% \subsubsection{Baseline}
% \begin{itemize}
%     \item Train a model on $S$ and $L$ jointly.
%     \item Measure performance on each corresponding validation set.
% \end{itemize}

% \subsubsection{Scale-specific NAS}
% \begin{itemize}
%     \item Train a model $f_S$ on $S$.
%     \item Train a model $f_L$ on $L$.
%     \item Compare the resulting architectures across, visualized in
%         Figure~\ref{fig:class-specific-nas-accuracy} and~\ref{fig:class-specific-nas-cell-count}:
%     \begin{itemize}
%         \item Multiple categories: \textit{car, person, bicycle}
%         \item Multiple runs, with different random seed.
%     \end{itemize}
% \end{itemize}

% \subsection{Analyzing Dynamic properties}
% \subsubsection{Problems with the original formulation}
% Refer to Figure~\ref{fig:class-specific-nas-cell-count}, where the variance across the whole dataset is plotted by the errorbar.
% \textbf{No variance} in Dynamic Routing~\cite{li2020learning} regardless which scales have been present during training time.
% Our hypothesis is that because there is no terms in the loss that would explicitly incentivize the gates to avoid mode collapse
% they fail to learn any useful data-dependent behaviour.
% On the other hand we see that the gates are actually trainable as they otpimize the budget constraint by finding a trivial solution
% that has low expected GFLOP value.
% In order to ensure the dynamic behaviour we employ Magnet Loss and then generalize the idea to its unsupervised alternative,
% which we refer to as deep clustering.

% \subsubsection{Enforcing Manual architecture design}
% \subsubsection{Supervised Dynamic model (i.e. Magnet Loss)}
% \subsubsection{Unsupervised Dynamic model (i.e. Deep Cluster)}

==> sections/motivation.tex <==
\section{Motivation}
\label{sec:motivation}
% \begin{table}[t]
% \centering
% \begin{tabular}{@{}lc@{\hskip 0.3in}c@{\hskip 0.3in}c@{}}
% \toprule
% Training & $\text{Accuracy} (\textrm{val}_S$) & \text{Accuracy} ($\textrm{val}_L$) & GFLOPs  \\ \midrule
% \textbf{S}: Small scale & 92.7 & 78.3 & 32.8 \\
% \textbf{L}: Large scale & 82.2 & 90.2 & 31.4 \\
% \textbf{X}: Mixed scale & 89.0 & \textbf{91.0} & 32.4
% \\ \bottomrule
% \textbf{X}: Supervised-DivDR & 91.1 & 88.3 & 31.0 \\
% \textbf{X}: DivDR & \textbf{93.1} & 83.0 & \textbf{28.2} \\
% \bottomrule
% \end{tabular}
% \caption{\textcolor{red}{UPDATED: The new results are not supporting the caption.}Comparison in accuracy and FLOPs on the ``car" class of cityescapes between local experts trained on specific subsets ($\textbf{S}$ and $\textbf{L}$) against a global expert trained on $\textbf{X}$. Moreover, when the labels for each subset in $\textbf{X}$ is available, our Supervised-DivDR can correctly find a soft assignment to local expert for new unseen samples. Even when the labels of the local biases in $\textbf{X}$ are not provided, DivDR can learn such local biases and find the correct soft assignment to local experts for new unseen samples.}
% \label{tab:motivatio_exps}
% \end{table}




\begin{table}[t]
\centering
\begin{tabular}{@{}lc@{\hskip 0.3in}c@{\hskip 0.3in}c@{}}
\toprule
Training & $\text{Accuracy} (\textrm{val}_S$) & \text{Accuracy} ($\textrm{val}_L$) & GFLOPs  \\ \midrule
\textbf{S}: Small scale & \textbf{92.84} & 82.04 & 32.75 \\
\textbf{L}: Large scale & 85.25 & \textbf{91.17} & 31.79 \\
\textbf{X}: Mixed scale & 90.87 & 90.92 & 32.33 \\ \midrule
% \textbf{X}: Supervised-DivDR & 91.21  & 90.64 & 32.25\\
\textbf{X}: DivDR & 91.79 & 90.02 & \textbf{31.40}  \\
\bottomrule
\end{tabular}
\caption{
Comparison in accuracy and FLOPs on the ``car" class of Cityscapes~\cite{cordts2016cityscapes} between local experts trained on specific subsets ($\textbf{S}$ and $\textbf{L}$) against a global expert trained on $\textbf{X}$.
We used DR~\cite{li2020learning} framework to obtain the expert models.
Furthermore, we report our proposed method, DivDR's performance.
Scores are averaged over 3 identical runs with different seeds.
FLOPs are averaged over the two validation set.
}
\label{tab:motivatio_exps}
\end{table}









% \begin{table}[t]
% \centering
% \caption{
%     Comparison between models trained with different levels of supervision.
%     The \textit{Oracle} refers to a hypothetical model derived from Table~\ref{tab:local-vs-global} where the experts are assigned correctly for every image during inference time
% }
% \begin{tabular}{@{}lcccc@{}}
% \toprule
% Method & Accuracy ($\textrm{val}_S$) & Accuracy ($\textrm{val}_L$) & GFLOPs & Accuracy ($S$ vs. $L$) \\ \midrule
% % Oracle & 93.6 & 95.0 & avg(63.9, 48.4) & 100.0\% \\
% Supervised-DDR & 93.4 & 94.5 & 54.0 & 99.2\%  \\
% DDR &  91.0 & 92.7 & 51.3 & 98.1\% \\ \bottomrule
% \end{tabular}
% \label{tab:supervised}
% \end{table}


We first start by motivating our key hypothesis: \textit{``training \textit{local experts} on learnt subsets of the training data each sharing local biases can jointly outperform \textit{global experts}, i.e. models that were trained over the entire dataset"}. We motivate this on the task of semantic segmentation where we synthetically construct datasets each with a specific object scale bias. In particular, we only consider the ``car" class in the Cityscapes~\cite{cordts2016cityscapes} dataset and partition it into two subsets; one containing small scale cars denoted as \textbf{S} and the other containing large scale cars denoted as \textbf{L}. We then mix both subsets together into a subset named \textbf{X} to mimic a dataset with unknown subsets of biases. The technical details on the construction of each dataset is left for the \textbf{supplementary material}. We then train Dynamic Routing Networks \cite{li2020learning}, particularly Dynamic-A with the smallest computational budget, on the three curated datasets, i.e. \textbf{S}, \textbf{L}, and \textbf{X} and report the mIOU on the validation sets of \textbf{S} and \textbf{L} denoted as $\textrm{val}_{S}$ and $\textrm{val}_L$, respectively, in Table \ref{tab:motivatio_exps}. Moreover, we also report the computational complexity of each trained model measured in GLOPs on a fixed input image resolution for a fair comparison (see the \textbf{supplementary material} for details). As seen from Table \ref{tab:motivatio_exps}, \textit{local} experts outperform the \textit{global} expert (trained on \textbf{X}), in terms accuracy. That is to say, training a network on subsets of the data sharing similar local biases allows for better performing models when evaluated on the corresponding subset, e.g. trained on $\mathbf{S}$ and tested on $\textrm{val}_S$. Moreover, training one global expert on the mixed scale subset $\mathbf{X}$ results in a less efficient network with a correspondingly lower mIoU on each subset individually. Moreover, we visualize in Figure \ref{fig:s-l-x-arch} the trained models on each subset showing at which resolutions activations were processed. We observe that DR~\cite{li2020learning} trained on \textbf{S} (Figure \ref{fig:s-l-x-arch} right) results in networks using only high resolution activations (as depicted by thick arrows in the first row). This is as opposed to Dynamic-A trained on $\textbf{L}$ (Figure \ref{fig:s-l-x-arch} middle) where more activations are processed at their lower resolution as depicted by the thick arrows at bottom rows. On the contrary, when there is not explicit bias presented during training, the global expert trained on $\textbf{X}$ (Figure \ref{fig:s-l-x-arch} right), the trained network uses activation resolutions at all scales resulting in a less efficient and worse performing model.

In practice, such local biases are not available during training (Challenge (i)). Moreover, even if they were available during training, it remains unclear how to select the correct local expert for new unseen samples (Challenge (ii)). To address both problems jointly, we propose an unsupervised approach, dubbed DivDR, that learns the local biases during training (Challenge (i)) and performs a soft assignment to local experts for every new unseen example (Challenge (ii)). In Table \ref{tab:motivatio_exps}, we report both mIOU and the corresponding FLOPs for our approach trained on \textbf{X} and evaluated on both $\textrm{val}_S$ and $\textrm{val}_L$. 
DivDR learns the subsets of local biases and performs soft assignments for new unseen samples results in a marginal accuracy drop of only $2.4\%$ and $1.8\%$ on $\textrm{val}_S$ and $\textrm{val}_L$, respectively while maintaining an improved efficiency of $51.3$ GLOPs. Moreover, interestingly, we observe that the learnt subsets of DivDR overlaps by $98.1\%$ with $\textbf{S}$ and $\textbf{L}$ that are explicit in $\textbf{X}$. This demonstrates the capacity of DivDR to uncover in an unsupervised approach the local biases in the dataset. We now move to our proposed approach DivDR.


\input{figures/s-l-x-arch}

% We conclude that the \textit{test} time expert assignment problem can be solved without sacrificing accuracy, provided subset labels are available during \textit{training} time.
% However, dependency on such levels of supervision still poses an important challenge that we have to address.

% We note that there is only a marginal accuracy drop accuracy drop of 0.2\% and 0.5\% on $\text{val}_S$ and $\text{val}_L$, respectively with a slight improvement on FLOPs, 54 GLOPs as opposed 63.9 GLOPs and 48.4 GLOPs.



% Moreover, we alsWe also show that our proposed soft assignment procedure for when 



% To examine the role of assignment,  \textcolor{red}{Challenge (i)} 

% To address \textcolor{red}{Challenge (i)}, we train our proposed DDR where the labels for each subset \textbf{S} and \textbf{L} are provided during training time which we dub \textrm{Supervised-DDR}. Moreover, we also report the performance for DDR where the subsets are learnt in an unsupervised approach with the soft assignment of local experts for unseen new samples. We note that there is only a marginal accuracy drop accuracy drop of 0.2\% and 0.5\% on $\text{val}_S$ and $\text{val}_L$, respectively with a slight improvement on FLOPs, 54 GLOPs as opposed 63.9 GLOPs and 48.4 GLOPs. 

% that the average of both local experts trained on each subset seperately (54.0 GLOPs as opposed to 

% retained (an improvement of 2.2 GFLOPs).

% \textrm{supervised-DDR} is

% Note that the local experts from Table~\ref{tab:local-vs-global} are results of two individual training process, whereas the \textit{Supervised} model in Table~\ref{tab:supervised} is a result of a single training.
% Despite a marginal accuracy drop (0.2\% and 0.5\%) the efficiency of the \textit{Oracle} is retained (an improvement of 2.2 GFLOPs).

% We conclude that the \textit{test} time expert assignment problem can be solved without sacrificing accuracy, provided subset labels are available during \textit{training} time.
% However, dependency on such levels of supervision still poses an important challenge that we have to address.






% The differences between the resulting architectures are shown in Fig~\ref{fig:s-l-x-arch}.
% Note that the \textit{global expert} (on the \textit{right}) applies more cells and is less selective w.r.t. the resolution compared to (\textit{left} and \textit{middle}).
% On the other hand, the architecture learned for small objects (\textit{left}) learns to use more high resolution operations, whereas for large objects more low resolution nodes are activated.




% From the results, we conclude that the \textit{local} experts outperform the \textit{global} expert in terms of both efficiency and accuracy.
% This means that during test time if we know which expert to use, we can achieve better performance with less computation.


% However, this condition rarely holds in real life applications, therefore we address it by using Dynamic Routing Networks~\cite{li2020learning}.




% Note that each training is jointly optimizing the model accuracy and the model complexity (details discussed in Sec.~\ref{sec:method}).




% train three models 


% we train three models from identical initial state, one for each dataset: \textbf{S}, \textbf{L} and \textbf{X}.
% The results are shown in Table~\ref{tab:local-vs-global}.
% Note that each training is jointly optimizing the model accuracy and the model complexity (details discussed in Sec.~\ref{sec:method}).
% From the results, we conclude that the \textit{local} experts outperform the \textit{global} expert in terms of both efficiency and accuracy.
% This means that during test time if we know which expert to use, we can achieve better performance with less computation.
% However, this condition rarely holds in real life applications, therefore we address it by using Dynamic Routing Networks~\cite{li2020learning}.




% select a set of images containing objects of either large or small scale and label them as \textbf{L} and \textbf{S} dataset respectively.
% Followed by that, we mix the images from \textbf{L} and \textbf{S} into \textbf{X} to mimic an ``unlabeled" dataset that has significant hidden local bias.
% For details on the toy-dataset selection process, see the Supplementary Material~\ref{sec:toydata}.


% We first 

% We compare the performance of global experts against local experts.




% we start by constructing a toy dataset with a specifically chosen local bias, such that we can gradually relax the dependence of the trained models on such prior knowledge while monitoring the consequences of the relaxation under controlled circumstances.
% Using semantic segmentation as a surrogate downstream task, we compare the performance of global experts against local experts.
% Followed by that, we address the expert assignment problem and show that using subset-labels during \textit{training} time, we can select the corresponding local expert with high accuracy during \textit{test} time.
% Finally, we show how can we use iterative clustering to recover subset-labels without relying on external supervision.

% \subsection{Dataset generation}
% To illustrate the differences between local and global experts we use object scale as an anchor for subset bias, as it is fairly easy to gather such statistics from any dataset that has object level annotation.
% We carefully select a set of images containing objects of either large or small scale and label them as \textbf{L} and \textbf{S} dataset respectively.
% Followed by that, we mix the images from \textbf{L} and \textbf{S} into \textbf{X} to mimic an ``unlabeled" dataset that has significant hidden local bias.
% For details on the toy-dataset selection process, see the Supplementary Material~\ref{sec:toydata}.

% \subsection{Global vs. local experts}
% Followed by the data generation, we train three models from identical initial state, one for each dataset: \textbf{S}, \textbf{L} and \textbf{X}.
% The results are shown in Table~\ref{tab:local-vs-global}.
% Note that each training is jointly optimizing the model accuracy and the model complexity (details discussed in Sec.~\ref{sec:method}).
% From the results, we conclude that the \textit{local} experts outperform the \textit{global} expert in terms of both efficiency and accuracy.
% This means that during test time if we know which expert to use, we can achieve better performance with less computation.
% However, this condition rarely holds in real life applications, therefore we address it by using Dynamic Routing Networks~\cite{li2020learning}.

% \input{figures/s-l-x-arch}

% The differences between the resulting architectures are shown in Fig~\ref{fig:s-l-x-arch}.
% Note that the \textit{global expert} (on the \textit{right}) applies more cells and is less selective w.r.t. the resolution compared to (\textit{left} and \textit{middle}).
% On the other hand, the architecture learned for small objects (\textit{left}) learns to use more high resolution operations, whereas for large objects more low resolution nodes are activated.


% \subsection{Expert assignment using Dynamic Networks}
% In order to utilize local experts during test time we have to make the model architecture $\mathcal{A}$ dependent on the input image $\mathcal{A}=\mathcal{A}(x)$.
% As we discussed in Sec.~\ref{sec:related}, the main question is how do we implement such models.
% The most generic approach is to decouple $\mathcal{A}(x)=\sum\sigma_{i}\circ \mathcal{A}_{i}(x)$, where $\mathcal{A}_i$ is the local expert and $\sigma_i$ is the gating \csabir{or selection, or hypernetwork} function.
% The key concept is that the gating mechanism is responsible for selecting only the most relevant experts to be evaluated, based on the input of the experts, to reduce computational costs.

% While some approaches implement gating by using an external, computationally intensive model, we use Dynamic Routing Networks~\cite{li2020learning}, because of their efficient gate function design, as it reuses the same features computed by the previous layers.
% \csabir{Maybe it would be useful here to drop some notation that can be reused in 3.4}
% Extending the original objective function of~\cite{li2020learning} with a term that encourages the network to learn distinct layouts for different subsets, we train a model that can assign the correct local expert during test time with 99.2\% accuracy.
% The results are shown in Table~\ref{tab:supervised} in the second row.
% Note that the local experts from Table~\ref{tab:local-vs-global} are results of two individual training process, whereas the \textit{Supervised} model in Table~\ref{tab:supervised} is a result of a single training.
% Despite a marginal accuracy drop (0.2\% and 0.5\%) the efficiency of the \textit{Oracle} is retained (an improvement of 2.2 GFLOPs).

% We conclude that the \textit{test} time expert assignment problem can be solved without sacrificing accuracy, provided subset labels are available during \textit{training} time.
% However, dependency on such levels of supervision still poses an important challenge that we have to address.

% \subsection{Learning subset labels from data}
% Statistics of a dataset might be provided by the creators (location, camera parameters etc.), potentially can be inferred from the labels (e.g. object density, scales, poses etc.) or even the images themselves (lighting conditions, appearance etc.) as part of the pre-process, as e.g. done in~\cite{mullapudi2018hydranets}.
% However, arbitrarily picking one aspect to categorize and partition a dataset might be disadvantageous, and often times impractical as the subset level labels are not available.

% In the space of architectures $\{A\}$, spanned by the gating scores $\sigma$ of Dynamic Routing~\cite{li2020learning}, we use \textit{magnet loss}~\cite{rippel2015metric}, an iterative $K$-means clustering technique to learn a partitioning of the dataset
% that corresponds to the most distinct architectures.
% \csabir{definitely needs to be clarified. but how?}
% Later on we use the resulting cluster centers $\mu$ to assign the datapoints to different subsets.
% The assignment steps are illustrated in Fig.~\ref{fig:kmeans}.
% Furthermore, between the subsequent $K$-means updates, we train our model in similar fashion to the \textit{Supervised} approach using the labels obtained from the clustering as supervision.

% The corresponding results are shown in the last row of Table~\ref{tab:supervised}.
% With the removal of subset level supervision the experts were trained on changing \csabir{evolving?} partitions of the data, that results in  further drop in accuracy (2.6\% and 2.3\% respecitvely), however the accuracy w.r.t. the original subset labels reached a staggering 98.1\%.

% This result is encouraging because it means that if any hidden local dataset bias is present the \textit{Unsupervised} method can recover the latent subset labels (only assuming the number of clusters $K$)




==> tables/centroid-update.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{l|lllllll}
    \textbf{centroid update} & \textbf{5} & \textbf{10} & \textbf{20} & \textbf{50} & \textbf{100} & \textbf{250} & \textbf{1000} \\ \hline
    intra-distance           &            &             &             &             &              &              &               \\
    inter-distance           &            &             &             &             &              &              &
    \end{tabular}
\caption{Comparison on varying the update frequency of the $k$-mean cluster centers.}
\label{tab:centroid-update}
\end{table}

==> tables/cityscapes-inter-intra.tex <==
\begin{table}[ht]
\centering
\caption{Quantitative analysis of semantic segmentation on Cityscapes~\cite{cordts2016cityscapes}. We report \textit{Inter} and \textit{Intra} cluster variance, that shows how far are the cluster centers are from each other in $L_2$ space and how close are the samples to the cluster centers respectively.}
\begin{tabular}{@{}l@{\hskip 0.1in}l@{\hskip 0.1in}c@{\hskip 0.1in}l@{\hskip 0.1in}c@{}}
\toprule
\textbf{method} & \textbf{mIoU} & \textbf{FLOPs} & \textbf{Inter} & \textbf{Intra} \\ \midrule
Dyn-A & 72.7 & 58.7 & 0.4 & 0.3 \\
Ours Constrained & 72.0 & 49.9 & 0.6 & 0.2 \\
Dyn-R & 75.2 & 99.2 & 1.5 & 1.5 \\
Our Unconstrained & 75.7 & 98.3 & 1.2 & 0.5 \\ \bottomrule
\end{tabular}
\end{table}

==> tables/cityscapes.tex <==
\begin{table*}[t]
\centering
\caption{
    Comparison with baselines on the Cityscapes~\cite{cordts2016cityscapes} validation set.
    * Scores from~\cite{li2020learning} were reproduced using the \href{https://github.com/Megvii-BaseDetection/DynamicRouting}{official implementation}.
    The evaluation settings are identical to~\cite{li2020learning}.
    We calculate the average FLOPs with $1024\times 2048$ size input.
}
\begin{tabular}{lc@{\hskip 0.1in}l@{\hskip 0.1in}r}
\toprule
\textbf{Method}           & \textbf{Backbone}          & \textbf{$\mathbf{mIoU}_{val}(\%)$} & \textbf{GFLOPs} \\ \midrule
BiSenet~\cite{yu2018bisenet}          & ResNet-18         & 74.8                      & 98.3   \\
DeepLabV3~\cite{chen2017rethinking}        & ResNet-101-ASPP   & 78.5                      & 1778.7 \\
Semantic FPN~\cite{kirillov2019panoptic}     & ResNet-101-FPN    & 77.7                      & 500.0  \\
DeepLabV3+~\cite{chen2018encoder}       & Xception-71-ASPP  & 79.6                      & 1551.1 \\
PSPNet~\cite{zhao2017pyramid}           & ResNet-101-PSP    & 79.7                      & 2017.6 \\
Auto-DeepLab~\cite{liu2019auto}    & Searched-F20-ASPP & 79.7                      & 333.3  \\
Auto-DeepLab~\cite{liu2019auto}    & Searched-F48-ASPP & 80.3                      & 695.0  \\ \midrule
DR-A~\cite{li2020learning}* & Layer16           & 72.7$\pm$0.6                     & 58.7$\pm$3.1       \\
DR-B~\cite{li2020learning}* & Layer16           & 72.6$\pm$1.3                     & 61.1$\pm$3.3       \\
DR-C~\cite{li2020learning}* & Layer16           & 74.2$\pm$0.6                    & 68.1$\pm$2.5       \\
DR-Raw~\cite{li2020learning}* & Layer16           & 75.2$\pm$0.5                     & 99.2$\pm$2.5        \\ \midrule
DivDR-Raw  & Layer16           &  75.4$\pm$1.6          & 95.7$\pm$0.9      \\
DivDR-A    & Layer16           &  73.5$\pm$0.4           & 57.7$\pm$3.9       \\
\bottomrule
\end{tabular}
\label{tab:full-cityscapes-comp}
\end{table*}

==> tables/coco-k.tex <==
\begin{table}[ht]
\caption{
Quantitative comparison of Dynamic Routing~\cite{li2020learning} trained without the objective to diversify the paths and using various $K$ for the clustering term. We omit $K=1$ from our results as it reverts to forcing the model to use the same architecture, independent of the input image.
For comparison we report best Dynamic Routing~\cite{li2020learning} scores from 3 identical runs with different seeds
}
\begin{subtable}{.5\linewidth}
    \caption{Constrained}
    \centering
    \begin{tabular}{@{}r@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c@{}}
    \toprule
    \textbf{K} & \textbf{mAP}$_{val}$ & \textbf{GFLOPs} & \textbf{Inter} & \textbf{Intra} \\ \midrule
    * & 34.6 & 23.2 & 0.2 & 0.3 \\
    2 & \textbf{35.1} & 21.9 & 1.1 & 0.4 \\
    3 & 35.0 & \textbf{19.2} & 0.8 & 0.3 \\
    4 & 34.9 & 20.0 & 0.6 & 0.1 \\ \bottomrule
    \end{tabular}
\end{subtable}
\begin{subtable}{.5\linewidth}
    \caption{Unconstrained}
    \centering
    \begin{tabular}{@{}r@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c@{\hskip 0.1in}c@{}}
    \toprule
    \textbf{K} & \textbf{mAP}$_{val}$ & \textbf{GFLOPs} & \textbf{Inter} & \textbf{Intra} \\ \midrule
    * & 37.8 & 38.2 & 0.5 & 0.7 \\
    2 & 36.5 & \textbf{31.0} & 0.6 & 0.5 \\
    3 & 37.4 & 32.6 & 1.2 & 0.5 \\
    4 & \textbf{38.1} & 32.8 & 0.7 & 0.2 \\ \bottomrule
    \end{tabular}
\end{subtable}
\end{table}

==> tables/dr-idr-toy.tex <==
% \begin{table*}[h]
%     \label{tab:dr-idr-toy}
%     \centering
%     \begin{tabular}{ccccccc}
%     \toprule
%     \textbf{Method}          & $\mathcal{D}_S$ & $\mathcal{D}_L$ & $\mathcal{D}_X$ & $\mathrm{IoU}^{\mathcal{D}_S}_{val}(\%)$ & $\mathrm{IoU}^{\mathcal{D}_L}_{val}(\%)$ & GFLOPs \\ \midrule
%     DR~\cite{li2020learning} & \checkmark      &                 &                 & 93.6                                      &              89.6                        & 63.9   \\
%     DR~\cite{li2020learning} &                 & \checkmark      &                 &          60.7                                 & 95.0                           & 48.4    \\
%     DR~\cite{li2020learning} &                 &                 & \checkmark      & 68.7                                      & 83.1                                      & 76.9   \\ \midrule
    
%     % CS-NAS + Oracle$\dagger$          & \checkmark      & \checkmark      &                 & 93.6                             & 95.0                                      & 56.2 $+c$      \\ 
%     iDR-supervised (ours)    & \checkmark      & \checkmark      &                 & 93.4                                      & 94.5                                     & 54.0   \\
%     iDR-unsuperv. (ours)     &                 &                 & \checkmark      & 91.0                                      & 92.7                                & 51.3     \\ \bottomrule
%     \end{tabular}
% \caption{
%     Comparisons with the original formulation of DR~\cite{li2020learning} and our improved routing mechanism iDR on the scale-specific toy experiment, derived from the Cityscapes dataset.
%     For both DR~\cite{li2020learning} and iDR, we report the best results out of 3 runs with different random seeds.
%     % \emph{CS-NAS + Oracle} refers to the hypothetical setup where we assume that the routing task is carried out by an external module that provides the source label of the validation set samples in $+c$ operations.
% }
% \end{table*}

==> tables/dr-std.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h]
    \label{tab:dr-std}
    \centering
    \begin{tabular}{@{}cccc@{}}
    \toprule
    \textbf{Train / Val} & $\mathcal{D}_S$ & $\mathcal{D}_L$ & $\mathcal{D}_X$ \\ \midrule
    $\mathcal{D}_S$  & 4.9 & 6.1 & 6.0 \\ 
    $\mathcal{D}_L$  & 4.2 & 4.2 & 4.5 \\
    $\mathcal{D}_X$  & 2.3 & 2.2 & 2.3 \\ \midrule
    iDR-supervised   & 0.9 & 1.2 & 2.4 \\
    iDR-unsupervised & 1.8 & 1.4 & 6.8 \\ \bottomrule
    \end{tabular}
    \caption{
        We report the average of the standard deviation scores ($\times 10^4$) over three DR~\cite{li2020learning} models, trained with different random seeds.
        From these results, we conclude that the model trained with the original DR~\cite{li2020learning} formulation is not dynamic.
        % In the Appendix%~\ref{appendix:dynamic-is-static} we show that each run results in different architectures while achieving the same accuracy.
    }
\end{table}

==> tables/img-per-update.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|ccccccccc}
    \textbf{centroid update} & \multicolumn{3}{c}{\textbf{5}}    & \multicolumn{3}{c}{\textbf{20}}   & \multicolumn{3}{c}{\textbf{100}} \\
    batches per update  & 5 & 20 & \multicolumn{1}{c|}{100} & 5 & 20 & \multicolumn{1}{c|}{100} & 5        & 20        & 100       \\ \hline
    intra-distance           &   &    &                          &   &    &                          &          &           &           \\
    inter-distance           &   &    &                          &   &    &                          &          &           &
    \end{tabular}
    \caption{
        Comparison of how many images to compute the $k$-means over.
        The images are sampled from the same pool as the training data is sampled from.
        More specifically the samples are drawn in the same order as the training samples,
        which means that if the \emph{centroid update period} matches the \emph{batches used for each update},
        the cluster centers are computed over the very same samples that the objective function will be optimized over after the update.
    }
    \label{tab:img-per-update.tex}
\end{table}

==> tables/num-clusters.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{c|cccc}
    \textbf{\# Clusters}      & 2 & 3 & 5 & 7 \\ \hline
    $\mathrm{mIoU}_{val}(\%)$ &   &   &   &   \\
    GFLOPs                    &   &   &   &
    \end{tabular}
\caption{Comparison of number of clusters in terms of accuracy and model complexity.}
\label{tab:num_clusters}
\end{table}
